The continuous weak order

The set of permutations on a finite set can be given the lattice structure known as the weak Bruhat order. This lattice structure is generalized to the set of words on a fixed alphabet $\Sigma$ = {x,y,z,...}, where each letter has a fixed number of occurrences. These lattices are known as multinomial lattices and, when card($\Sigma$) = 2, as lattices of lattice paths. By interpreting the letters x, y, z, . . . as axes, these words can be interpreted as discrete increasing paths on a grid of a d-dimensional cube, with d = card($\Sigma$).We show how to extend this ordering to images of continuous monotone functions from the unit interval to a d-dimensional cube and prove that this ordering is a lattice, denoted by L(I^d). This construction relies on a few algebraic properties of the quantale of join-continuous functions from the unit interval of the reals to itself: it is cyclic $\star$-autonomous and it satisfies the mix rule.We investigate structural properties of these lattices, which are self-dual and not distributive. We characterize join-irreducible elements and show that these lattices are generated under infinite joins from their join-irreducible elements, they have no completely join-irreducible elements nor compact elements. We study then embeddings of the d-dimensional multinomial lattices into L(I^d). We show that these embeddings arise functorially from subdivisions of the unit interval and observe that L(I^d) is the Dedekind-MacNeille completion of the colimit of these embeddings. Yet, if we restrict to embeddings that take rational values and if d > 2, then every element of L(I^d) is only a join of meets of elements from the colimit of these embeddings.

==> macros.tex <==
\RequirePackage{ifthen}

\RequirePackage[boxsize={3mm},tabloids=off]{ytableau}
\RequirePackage{rotating}
\RequirePackage{amsmath,amssymb}
\newcommand{\tand}{\text{ and }}
\newcommand{\tiff}{\text{ iff }}
\newcommand{\timplies}{\text{ implies }}
\newcommand{\toth}{\text{ otherwise }}
\newcommand{\ttoth}{\text{otherwise}}
\RequirePackage{txfonts}
\RequirePackage[all]{xy}
\RequirePackage{tikz-cd}

\RequirePackage{hyperref}

\newenvironment{prop}{\vskip 6pt\par\noindent{\bf Proposition.~\em}}{\par\vskip 6pt}

\newenvironment{thm}{\vskip 6pt\par\noindent{\bf Theorem.~\em}}{\par\vskip 6pt}

\RequirePackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{fact}{Fact}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{claim}{Claim}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}


\RequirePackage{xspace}
\newcommand{\staraut}{$\star$-autonomous\xspace}
\newcommand{\saq}{\staraut quantale\xspace}
\newcommand{\msaq}{mix \staraut quantale\xspace}
\newcommand{\bs}{bisemigroup\xspace}
\newcommand{\Bs}{bi-semigroup\xspace}
\newcommand{\bm}{bimonoid\xspace}
\newcommand{\lbs}{$\ell$-\bs}
\newcommand{\lbm}{$\ell$-\bm}
\newcommand{\Lbs}{lattice-ordered \Bs}
\newcommand{\LBS}{Lattice-ordered \Bs}
\newcommand{\U}[1]{\mid#1\mid}
\newcommand{\opp}[1]{{#1}^{\star}}
\newcommand{\Opp}[1]{#1^{\star}}
\newcommand{\OPP}[1]{#1{}^{\star}}
\newcommand{\opprj}[1]{\Joinof{\Radj{#1}}}
\newcommand{\oppml}[1]{\Ladj{\Meetof{#1}}}
\newcommand{\Star}[1]{{#1}^{\star}}

\newcommand{\funFiller}{-}
\newcommand{\oppopp}[1]{{#1}^{\star\star}}
\newcommand{\oppfun}{\opp{(\funFiller)}}
\newcommand{\secRef}[1]{Section~\ref{sec:#1}}


\newcommand{\qQ}{\mathcal{Q}}
\newcommand{\cL}{\mathcal{L}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\In}[1][n]{\I_{#1}}
\renewcommand{\Im}{\In[m]}

\renewcommand{\L}{\mathsf{L}}
\newcommand{\LI}[1][]{\L(\I^{#1})}
\newcommand{\LId}{\LI[d]}

\newcommand{\LRId}[1][d]{\L_{\mathcal{R}}(\I^{#1})}
\newcommand{\JR}{J_{\mathcal{R}}}
\newcommand{\Lf}{\L_{\mathfrak{f}}}
\newcommand{\LfI}{\Lf(\I)}
\newcommand{\LfId}{\LRId}

\newcommand{\Q}{\mathsf{Q}}
\newcommand{\Qj}{\Q_{\vee}}
\newcommand{\Qm}{\Q_{\land}}
\newcommand{\Lj}{\Q_{\vee}}
\newcommand{\LjI}{\Lj(\I)}
\newcommand{\QjI}{\Qj(\I)}
\newcommand{\Lm}{\Q_{\land}}
\newcommand{\LmI}{\Lm(\I)}


\newcommand{\meetof}[1]{{#1}^{\land}}
\newcommand{\joinof}[1]{{#1}^{\vee}}
\newcommand{\meetofjoinof}[1]{{#1}^{\vee\land}}
\newcommand{\joinofmeetof}[1]{{#1}^{\land\vee}}

\newcommand{\Meetof}[1]{#1^{\land}}
\newcommand{\MeetOf}[1]{\Meetof{#1}}
\newcommand{\MEETOF}[1]{#1{}^{\land}}
\newcommand{\Joinof}[1]{#1^{\vee}}
\newcommand{\JoinOf}[1]{\Joinof{#1}}
\newcommand{\JOINOF}[1]{#1{}^{\vee}}

\newcommand{\ladj}[1]{{#1}_{\ell}}
\newcommand{\radj}[1]{{#1}_{\rho}}
\newcommand{\Ladj}[1]{#1_{\ell}}
\newcommand{\Radj}[1]{#1_{\rho}}
\newcommand{\LADJ}{left adjoint\xspace}
\newcommand{\RADJ}{right adjoint\xspace}

\newcommand{\continuous}{continuous\xspace}
\newcommand{\jcont}{join-\continuous}
\newcommand{\jc}{\jcont}
\newcommand{\mcont}{meet-\continuous}
\newcommand{\mc}{\mcont}
\newcommand{\bcont}{bi-\continuous}
\newcommand{\bc}{\bcont}
\newcommand{\tcont}{topologically \continuous}

\newcommand{\rto}{\xrightarrow{\;\;}}
\newcommand{\rTo}{\rto}
\newcommand{\lrimpl}{\multimap}
\newcommand{\rlimpl}{\multimapinv}

\newcommand{\prodd}[2][d]{{#2}^{\couples{#1}}}
\newcommand{\PrLQ}{\prodd{Q}}
\newcommand{\PrdQ}{\prodd{Q}}
\newcommand{\PrLI}[1][d]{\prodd[#1]{\LjI}}


\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\cl}[1]{\closure{#1}}
\newcommand{\interior}[1]{#1^{\circ}}
\renewcommand{\int}[1]{\interior{#1}}
\newcommand{\set}[1]{\{\,#1\,\}}
\newcommand{\two}{{\bf 2}}
\newcommand{\Ld}[2][d]{\L_{#1}(#2)}

\newcommand{\Id}[1][d]{\I^{d}}
\newcommand{\p}{\mathsf{p}}
\newcommand{\IQ}{\I \cap \mathbb{Q}}
\newcommand{\card}{\mathrm{card}}

\newcommand{\setof}[1]{[#1]}
\newcommand{\setd}{\ensuremath{\setof{d}}}
\newcommand{\setn}{\ensuremath{\setof{n}}}
\newcommand{\setnp}{\ensuremath{\setof{n}_{+}}}
\newcommand{\setp}[1]{\ensuremath{\setof{#1}_{+}}}
\newcommand{\couples}[1]{\setof{#1}_{2}}
\newcommand{\cd}{\couples{d}}
\newcommand{\lin}[1]{To be defined}
\newcommand{\chp}[1]{\setof{#1}_{+}}
\newcommand{\osf}{one step function\xspace}
\newcommand{\ji}[1]{e_{#1}}
\newcommand{\mi}[1]{m_{#1}}
\newcommand{\Ji}[1]{\MeetOf{\ji{#1}}}
\newcommand{\JI}[1]{E_{#1}}
\newcommand{\jp}{join-prime\xspace}
\renewcommand{\mp}{meet-prime\xspace}
\newcommand{\cjp}{completely \jp}
\newcommand{\jirr}{join-irreducible\xspace}
\newcommand{\mirr}{meet-irreducible\xspace}
\newcommand{\Mirr}{Meet-irreducible\xspace}
\newcommand{\cjirr}{completely \jirr}
\newcommand{\Fam}[1]{\langle \,#1 \,\rangle}
\newcommand{\mji}[1]{\mu^{\vee}_{#1}}
\newcommand{\Mji}[1]{M^{\vee}_{#1}}
\newcommand{\dimmi}{\dim^{\land}}
\newcommand{\dimji}{\dim^{\vee}}
\newcommand{\mmi}{\mu^{\land}}
\newcommand{\Mmi}{M^{\land}}
\newcommand{\Mi}[4]{M^{#3,#4}_{#1,#2}}
\newcommand{\JJi}[4]{E^{#3,#4}_{#1,#2}}


\newcommand{\eofclaim}{\hfill\qed~{\it Claim}\par}
\newcommand{\resp}{resp.,\xspace}
\newcommand{\covered}{\prec}
\newcommand{\wBo}{weak Bruhat order\xspace}
\newcommand{\wo}{weak order\xspace}
\newcommand{\cwBo}{continuous \wBo}
\newcommand{\cwo}{continuous \wo}

\newcommand{\DMNc}{Dedekind-MacNeille completion\xspace}
\newcommand{\appr}[1][v]{\mathtt{appr}_{#1}}

\newcommand{\Associahedra}{associahedra\xspace}
\newcommand{\Permutohedra}{permutohedra\xspace}
\newcommand{\Permutohedron}{permutohedron\xspace}

\newcommand{\ie}{i.e.\xspace}
\newcommand{\F}[1]{E_{#1,1}}
\newcommand{\G}[1]{E_{0,#1}}

\newcommand{\myvec}[1]{|#1|}
\newcommand{\Jc}{\mathsf{Jc}}
\renewcommand{\Mc}{\mathsf{Mc}}
\newcommand{\CL}{CL}
\newcommand{\inter}{}
\newcommand{\vij}{}
\newcommand{\uij}{}
\newcommand{\floor}[1]{\left \lfloor{#1}\right \rfloor}
\newcommand{\f}{\mathsf{f}}
\newcommand{\iso}{\equiv}

\newcommand{\mydiagram}[2][]{\framebox#1{\begin{turn}{90}\ydiagram{#2}\end{turn}}}
\newcommand{\mytdiagram}[2][]{\framebox#1{\begin{turn}{180}\ydiagram{#2}\end{turn}}}

\newcommand{\Ri}[1][\iota]{R_{#1}}

\newcommand{\perfect}{perfect\xspace}
\newcommand{\lbisemigroup}{$\ell$-bisemigroup\xspace}
\newcommand{\nc}{non-commutative\xspace}
\newcommand{\bd}{bounded\xspace}
\newcommand{\rl}{residuated lattice\xspace}
\newcommand{\irl}{involutive \rl}

\newcommand{\lattsig}{\bot,\vee,\top,\land}
\newcommand{\tbd}[1]{\red{#1\footnote{\red{To be defined in firts
        section}}}}

\renewcommand{\leqslant}{\leq}
\renewcommand{\nleqslant}{\not\leq}

\newcommand{\lpoint}[1]{\draw (#1) node[circle,fill,blue, inner sep = 1pt] (){}}
\newcommand{\rpoint}[1]{\draw (#1) node[circle,fill,red, inner sep = 1pt] (){}}
\newcommand{\bpoint}[1]{\draw (#1) node[circle,fill,black, inner sep = 2pt] (){}}

\newcommand{\Perm}{{\mathcal{P}}}
\newcommand{\mirrd}[1]{[ #1 ]}
\newcommand{\jirrd}[1]{\langle #1 \rangle}
\newcommand{\cF}{\mathcal{F}}

\newcommand{\bigveeQjIcd}{\bigvee{\textstyle{{\!\!}_{\QjI^{\cd}}}}}



